The Hubble Deep Hydrogen Alpha (HDH$\alpha$) Project: I. Catalog of Emission-line Galaxies

We present the first results of the Hubble Deep Hydrogen Alpha (HDH$\alpha$) project, which analyzes the space-borne deep H$\alpha$ narrowband imaging data in the GOODS-S region. The HDH$\alpha$ data comprises 72 orbits' images taken with the HST ACS/WFC F658N filter. The exposure time varies across a total area of $\sim$76.1 $\rm{arcmin}^2$, adding up to a total exposure time of 195.7 ks, among which 68.8 ks are spent in the deepest region. These images are aligned, reprojected, and combined to have the same pixel grid as the Hubble Legacy Fields (HLF). The scientific goals of the HDH$\alpha$ include establishing a sample of emission-line galaxies (ELGs) including [O III] emitters at $z\sim$ 0.3, [O II] emitters at $z\sim$ 0.8, and Lyman-$\alpha$ emitters (LAEs) at $z \sim 4.4$, studying the line morphology of ELGs with high resolution imaging data, and statistically analyzing the line luminosity functions and line equivalent-width distributions of ELGs selected with HST. Furthermore, the HDH$\alpha$ project enhances the legacy value of the GOODS-S field by contributing the first HST-based narrowband image to the existing data sets, which includes the HST broadband data and other ancillary data from X-ray to radio taken by other facilities. In this paper, we describe the data reduction process of the HDH$\alpha$, select ELGs based on HST's F658N and broadband data, validate the redshifts of the selected candidates by cross matching with the public spectroscopic catalogs in the GOODS-S, and present a final catalog of the confirmed [O III] emitters at $z\sim$ 0.3, [O II] emitters at $z\sim$ 0.8, and LAEs at $z \sim 4.4$.

==> table/spectroscopic_catalog.tex <==
\setlength{\tabcolsep}{0.5mm}{
